Learning to Get Up

Getting up from an arbitrary fallen state is a basic human skill. Existing methods for learning this skill often generate highly dynamic and erratic get-up motions, which do not resemble human get-up strategies, or are based on tracking recorded human get-up motions. In this paper, we present a staged approach using reinforcement learning, without recourse to motion capture data. The method first takes advantage of a strong character model, which facilitates the discovery of solution modes. A second stage then learns to adapt the control policy to work with progressively weaker versions of the character. Finally, a third stage learns control policies that can reproduce the weaker get-up motions at much slower speeds. We show that across multiple runs, the method can discover a diverse variety of get-up strategies, and execute them at a variety of speeds. The results usually produce policies that use a final stand-up strategy that is common to the recovery motions seen from all initial states. However, we also find policies for which different strategies are seen for prone and supine initial fallen states. The learned get-up control strategies often have significant static stability, i.e., they can be paused at a variety of points during the get-up motion. We further test our method on novel constrained scenarios, such as having a leg and an arm in a cast.

==> discussion.tex <==
\section{Discussion}
% 1. distillation, 2. control of get-up style, 3. sit-to-stand?, 4. better character model? (to appendix)

The final policy trained by our framework~$\pi_{slow}$ needs to store the weak policy~$\pi_{weak}$ to generate reference trajectories. Thus, it requires a large memory footprint, limiting its usage in conditions with memory constraints. To mitigate this issue, we can distill $\pi_{slow}$ to a torque-based and pure state indexed policy via a teacher-student framework. Such distillation has been proven successful for some locomotion tasks on robots where data augmentation techniques are often found beneficial~\cite{lee2020learning, xie2018feedback}. The distilled policy no longer needs the weak policy~$\pi_weak$ to provide a reference trajectory. Furthermore, the distilled policy can contain a single velocity parameter to replace $\kappa$ as the speed control for the get-up motions. 

In this work, we show that our framework can explore diverse get-up motions without motion capture data. However, our method has little control over the style of the get-up motion. Ideally, the policy should adopt one optimal strategy to get up given the current situations. Instead, most controllers produced by our method often lock in one get-up strategy, and transform the current lying state to the preferred facing direction by rolling over on the ground to initiate the get-up motion. Current work still mainly learn physics-based motion controller subjected to style constraints with motion capture data~\cite{peng2021amp}. Control over style without motion capture data remains an exciting direction to explore in physics-based animation.

We focus on the get-up from the ground problem in this paper. Although getting up from the ground is common in daily life, other get-up problems are also of significant interest to solve. For example, humans also get up from various objects, such as chairs, sofas and bathtubs. Our framework can potentially solve those interesting variants because our framework is self-contained and does not rely on motion capture data. In addition, humans also can get up from irregular terrain. In the future, we also want to solve the get-up from various terrain problem with our framework by feeding the terrain information to the policy.
